My Face Is Mine, Not Yours: Facial Protection Against Diffusion Model Face Swapping

The proliferation of diffusion-based deepfake technologies poses significant risks for unauthorized and unethical facial image manipulation. While traditional countermeasures have primarily focused on passive detection methods, this paper introduces a novel proactive defense strategy through adversarial attacks that preemptively protect facial images from being exploited by diffusion-based deepfake systems. Existing adversarial protection methods predominantly target conventional generative architectures (GANs, AEs, VAEs) and fail to address the unique challenges presented by diffusion models, which have become the predominant framework for high-quality facial deepfakes. Current diffusion-specific adversarial approaches are limited by their reliance on specific model architectures and weights, rendering them ineffective against the diverse landscape of diffusion-based deepfake implementations. Additionally, they typically employ global perturbation strategies that inadequately address the region-specific nature of facial manipulation in deepfakes.

==> float/tikz-fig.tex <==
% \begin{figure}[t]
%     \centering
%     \resizebox{\linewidth}{!}{\begin{tikzpicture}[scale=0.7, transform shape,
%         node distance=1.8cm, auto,
%         block/.style={rectangle, draw, text centered, minimum width=1.8cm, minimum height=1cm, rounded corners},
%         arrow/.style={-{Stealth}, thick},
%         dashedarrow/.style={-{Stealth}, thick, dashed}
%       ]
      
%       % Main horizontal flow nodes (top branch)
%       \node (A) [block] {$x$};
%       \node (B) [block, right=2.0cm of A] {$z+\delta$};
%       \node (C) [block, right=2.0cm of B] {$z^\prime$};
%       \node (D) [block, right=1.0cm of C] {$x^\prime$};
%       \node (E) [block, right=2.3cm of D] {$c^\prime_{id}$};
%       \node (F) [block, right=2.3cm of E] {$\epsilon_\theta(z_t, t, c^\prime_{id})$};
%       \node (T) [block, right=1.0cm of F] {Target Img};
%       \node (adv) [block, below=4.cm of A] {$x_{\text{adv}}$};
      
%       % Branch: processing for c_{id} pathway from x (lower branch)
%       \node (G) [block, below=2.0cm of B] {$c_{id}$};
%       \node (I) [block, right=2.7cm of G] {$\epsilon_\theta(z_t, t, c_{id})$};
      
%       % Loss nodes merging the two paths
%       % Position L_ID beneath the midpoint between E (from the top branch) and G (from the lower branch).
%       \node (H) [block, right=2.7cm of I] {$L_{ID}$};
%       % Position L_avgDev beneath the midpoint between F and I.
%       \node (J) [block, right=2.7cm of H] {$L_{avgDev}$};
      
%       % Final node: Total_Loss, placed below the loss nodes.
%       \node (K) [block, below=1.8cm of $(H)!0.5!(J)$] {Total\_Loss};
      
%       % --- Insert image nodes above x and z+\delta ---
%       \node (imgA) [above=0.1cm of A] {\includegraphics[width=1.2cm]{Figs/sourceImg.png}};
%     %   \node (imgB) [above=0.1cm of B] {\includegraphics[width=1.2cm]{image_z.png}};
%       \node (imgTar) [above=0.1cm of T] {\includegraphics[width=1.2cm]{Figs/targetImg.jpg}};
%       \node (imgAdv) [above=0.1cm of adv]{\includegraphics[width=1.2cm]{Figs/advImg.jpg}};
      
%       % --- Draw arrows along the main horizontal chain ---
%       \draw [arrow] (A) -- node[midway, above] {$\mathcal{E}$} (B);
%       \draw [arrow] (B) -- node[midway, above] {SDEdit} (C);
%       \draw [arrow] (C) -- node[midway, above] {$\mathcal{D}$} (D);
%       \draw [arrow] (D) -- node[midway, above] {MLP $\circ$ ArcFace} (E);
%       \draw [arrow] (E) -- node[midway, above] {FaceAdapter} (F);
%       \draw [arrow] (T) -- node[midway, above] {} (F);
      
%       % --- Draw arrows for the lower branch ---
%       \draw [arrow] (A) -- node[midway, below left] {MLP $\circ$ ArcFace} (G);
%       \draw [arrow] (G) -- node[midway, above] {FaceAdapter} (I);
%       \draw [arrow] (T.south) to[out=-135, in=45] (I.north);
%       \draw [arrow] (B.south west) to[] node[near end, right] {$\mathcal{D}$} (adv.east);
      
%       % --- Draw merging arrows to the loss nodes using curved paths ---
%       \draw [arrow] (E.south) to[out=-90, in=45] (H.north east);
%       \draw [arrow] (G.north) to[out=30, in=145] (H.north west);
      
%       \draw [arrow] (F.south) to[out=-90, in=45] (J.north east);
%       \draw [arrow] (I.east) to[out=30, in=145] (J.north west);
      
%       % --- Connect the loss nodes down to Total_Loss ---
%       \draw [arrow] (H.south) to[out=-90, in=150] (K.north west);
%       \draw [arrow] (J.south) to[out=-90, in=30] (K.north east);
      
%       % --- Draw a dashed (curved) arrow for Gradient Update ---
%       \draw [dashedarrow] (K.west) to[bend left=45] node[midway, right] {Gradient Update} (B.south);
      
%       \end{tikzpicture}}
%     \caption{Pipeline of TODO}
%     \label{fig:enter-label}
% \end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figs/Piepline/Pipeline.pdf}
    \caption{Pipeline of TODO}
    \label{fig:enter-label}
\end{figure}
